Practical applications of metric space magnitude and weighting vectors

Metric space magnitude, an active subject of research in algebraic topology, originally arose in the context of biology, where it was used to represent the effective number of distinct species in an environment. In a more general setting, the magnitude of a metric space is a real number that aims to quantify the effective number of distinct points in the space. The contribution of each point to a metric space's global magnitude, which is encoded by the {\em weighting vector}, captures much of the underlying geometry of the original metric space. Surprisingly, when the metric space is Euclidean, the weighting vector also serves as an effective tool for boundary detection. This allows the weighting vector to serve as the foundation of novel algorithms for classic machine learning tasks such as classification, outlier detection and active learning. We demonstrate, using experiments and comparisons on classic benchmark datasets, the promise of the proposed magnitude and weighting vector-based approaches.

==> outline.tex <==
\section*{Outline}
FIXME: REMOVE ME!
\begin{enumerate}
    \item[abstract] (Glenn)
    \begin{enumerate}
        \item Introduce magnitude to the ML community
        \item Turns out that magnitude machinery can be used for boundary detection
        \item We can use it for classification
        \item Active learning for magnitude 
    \end{enumerate}
    \item[intro] (Dan, Eric, Jeff)
    \begin{enumerate}
        \item Intro to magnitude
        \begin{enumerate}
            \item history
            \item well-defined in arbitrary metric spaces. Could be applied to graphs.
            \item our focus is on Euclidean spaces
            \item connection to persistent homology
        \end{enumerate}
        \item Intro using magnitude for b,c,d from abstract (Dan, Glenn, Jeff)
        \item rest of the paper outline (Glenn)
    \end{enumerate}
    \item Interesting properties of magnitude
    \begin{enumerate}
        \item boundary detection (Jeff)
        \item Inclusion/exclusion (Eric)
        \item numerical considerations (schur complement) (Eric)
    \end{enumerate}
    \item Magnitude as a classifier (Dan)
    \begin{enumerate}
        \item define a classification task
        \item set up for the algorithm using magnitude
        \item algorithm
    \end{enumerate}
    \item  Magnitude for active learning (Glenn)
    \begin{enumerate}
        \item define active learning
        \item set up for magnitude for active learning
        \item algorithm
        \item cite Shur complement section
    \end{enumerate}
    \item Experiments on data sets (Dan, Eric)
    \begin{enumerate}
        \item classification; compare to other classification algorithms
        \item active learning; compare to random, uncertainty sampling; linear kernel
    \end{enumerate}
    \item conclusions and future work (Glenn, *)
\end{enumerate}

